Scalable Bayesian estimation in the multinomial probit model

The multinomial probit model is a popular tool for analyzing choice behaviour as it allows for correlation between choice alternatives. Because current model specifications employ a full covariance matrix of the latent utilities for the choice alternatives, they are not scalable to a large number of choice alternatives. This paper proposes a factor structure on the covariance matrix, which makes the model scalable to large choice sets. The main challenge in estimating this structure is that the model parameters require identifying restrictions. We identify the parameters by a trace-restriction on the covariance matrix, which is imposed through a reparametrization of the factor structure. We specify interpretable prior distributions on the model parameters and develop an MCMC sampler for parameter estimation. The proposed approach significantly improves performance in large choice sets relative to existing multinomial probit specifications. Applications to purchase data show the economic importance of including a large number of choice alternatives in consumer choice analysis.

==> notes.tex <==
PIATEK:
%user specified factor loadings based on structure choice categories, also increase linearly in number of categories. nested structure not available many applications. 

% With an increasing number
% of alternatives, however, it becomes prohibitively difficult to estimate. The proliferation
% of parameters in the covariance matrix implies that it is not only computationally
% challenging, but also difficult to interpret, because a large, unstructured covariance matrix
% is utterly non-informative about the unobserved heterogeneity that drives choices.

%contribute to factor model
%make suitable for mnp
%factor models used in mnp use outside info

Piatek p7: Contrary to traditional latent factor models where the factors are extracted from multiple manifest variables, in our framework only the choice is observed - a single categorical variable- and
the latent structure is obtained as the decomposition of the overall covariance matrix of
the model. No extra information is available to measure the latent factors, contrary to
integrated choice and latent variable (ICLV) models (Ben-Akiva et al., 2002; Bhat and
Dubey, 2014). This complicates both the identification and the inference of the model.
The fixed factor loadings structure we impose helps in this respect, as we will explain in
the following sections. 
(footnote: Estimating the factor loading matrix rather than fixing it would be possible in theory, but given the complexity of the task, we reserve this extension, and the investigation of its feasibility, for future research.)
WE DO NOT SOLVE THIS PROBLEM BY FIXING THE FACTOR LOADINGS, WE SOLVE THIS PROBLEM BY ONLY ESTIMATING THE LOADINGS AND DO NOT ESTIMATE THE FACTORS. HOW: BY ANGULAR DECOMPOSITION. DO NOT NEED FACTORS TO ESTIMATE LOADINGS, ONLY THE TRACE RESTRICTION.

setting:
decomposing the error terms of the utilities into latent factors and noise.
assume factor loadings, factors are latent.
contributions:
identification
computational-> MDA

Usually you sample the loadings conditional on the factors and sample the factors conditional on the loadings in eps=gamma*f+eta. Estimating both the factors and loadings in a multinomial model is difficult because we do not observe multiple utilities, but only one choice. Piatek et al solve this problem by fixing the factor loadings and sample the factors. We do not fix anything but only sample the factor loadings. The trick: using the angular system we can sample the loadings conditional on the trace (which has to be fixed anyway) instead of conditioning on factors. So we do not only use the angular trick for identification, but also to directly sample the loadings (without the need to sample factors). 

piatek: already know interpretation factors because of imposed nested structure.
argue that do not know a priori: for instance, in products can be health, luxury, shelf..


% \section{Likelihood and priors in literature}


% \subsection*{Likelihood function}
% Define the observed choices $y=(y_1,\dots,y_N)'$, and the likelihood is
% \begin{align}
%     p(y|\beta,\Sigma)=\prod_{i=1}^N \prod_{j=1}^J Pr[Y_i=j|\beta,\Sigma]^{I[y_i=j]},
% \end{align}
% where $I[.]$ is an indicator function and the probabilities are defined by
% \begin{align}
%     Pr[Y_i=j|&\beta,\Sigma] = \int_{-\infty}^{z_{ij}} \dots \int_{-\infty}^{z_{ij}} \int_{-\infty}^{z_{ij}} \dots \int_{-\infty}^{z_{ij}} (2\pi)^{-\frac{1}{2}J}|\Sigma|^{-\frac{1}{2}}\\&\exp\left( \frac{1}{2}(z_i-\beta x_i)'\Sigma^{-1}(z_i-\beta x_i)\right)dz_{i1}\dots dz_{ij-1} dz_{ij+1}\dots dz_{iJ}.
% \end{align}

% \subsection*{Complete data likelihood function}

% \begin{align}
%     p(y,Z|\beta,\Sigma)= \prod_{i=1}^N \prod_{j=1}^J  (2\pi)^{-\frac{1}{2}J}|\Sigma|^{-\frac{1}{2}}\exp\left( \frac{1}{2}(z_i-\beta x_i)'\Sigma^{-1}(z_i-\beta x_i)\right)\\I[y_i=j]I[z_{ij}>\max(z_{i1},\dots,z_{ij-1},z_{ij+1},\dots,z_{iJ})]
% \end{align}


%%%%%%%%%%%%%%%



% Summarize related literature.
% Multinomial probit models with factor structure
% \begin{itemize}
%     \item \citet{geweke1994alternative}: $\Sigma$ unrestricted, diagonal, identity. Make difference $\Sigma$ in unrestricted model and $\Sigma^*$ in differenced model explicit. covmat in undifferenced model is diagonal-> factor model in differenced model.
%     \item \citet{piatek2017multinomial}: Our methodological contribution is to develop a very general approach for cross-sectional data that relates a number of unobserved factors to the utilities of the alternatives. These (possibly correlated) factors can directly reflect an economic decision model and are not extracted from a measurement system, only assigned to the utilities through an allocation matrix.
% \end{itemize}

% \subsection*{Prior 1: fix element diagonal covariance matrix}
% Follow \citet{mcculloch2000bayesian} and specify
% \begin{align}
%   \Sigma &= \begin{bmatrix}
%     1 & \gamma' \\ \gamma & \Phi+\gamma \gamma',
%     \end{bmatrix},
%     \quad \gamma \sim N(b_{\gamma},B_{\gamma}),\quad \Phi^{-1}\sim W(c,C),\\ 
%     \beta_{2:J} &\sim N(b_{\beta},B_{\beta}),\quad \beta_1=0.
% \end{align}

% The scale is identified by setting the variance of a the base category, which is the first category, equal to 1. The location is identified by setting the coefficients corresponding to a base category, again category 1, equal to zero.

% The prior distribution specification is 
% \begin{align}
%     p(\beta,\Sigma) = p(\beta)p(\Sigma|\gamma,\Phi)p(\gamma)p(\Phi^{-1})
% \end{align}

% \subsection*{Prior 2: sum-to-zero restriction latent utilities}
% Follow \citet{burgette2019symmetric} (6 alternatives in applications) and specify
% \begin{align}
% \Sigma &= RR',\quad R = \begin{bmatrix} R_{1:(b-1)}\\R_b^*\\R_{b:J} \end{bmatrix},\quad R_b=[chol(\Sigma_b)]',\quad \Sigma_b \sim p_{TR}(S,\nu),\\ 
%     \beta&=f(\beta_b),\quad \beta_b\sim N(0,N_{\beta}),\\
%     b&\sim Unif({1,\dots,J}),
% \end{align}
% where the prior distribution of $\Sigma_b$ is
% \begin{align}
%     \Sigma_b \sim p_{TR}(S,\nu) \propto |\Sigma^*|^{-(\nu+J)/2}[tr(S\Sigma^{*-1})]^{-\nu(p-1)/2}I[tr(\Sigma^*)=p-1].
% \end{align}
% By restricting the trace of the covariance matrix, this distribution does not need a base category to identify the scale. 

% To make sure that also the identification of the location does not rely on a base category, this prior imposes a sum-to-zero restriction on the utilities. 
% The $R_b^*$ is a row vector inserted into $R_b$ at the $b$th row such that the sum of each column of R is zero. The function $f(\beta)$ is equal to $\beta$ with an element inserted into each $\beta_j$ at the $b$th row such that the sum of $\beta_j$ is zero.

% The prior distribution specification is 
% \begin{align}
%     p(\beta,\Sigma) = p(\beta|b)p(\Sigma|b)p(b)
% \end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Introduction to Bayesian factor analysis
%http://www.gatsby.ucl.ac.uk/~iam23/05jc/fa_talk.pdf
MODERN BAYESIAN FACTOR ANALYSIS
%http://hedibert.org/wp-content/uploads/2018/06/mbfa-lopes-2014.pdf
Fitting a Bayesian Factor Analysis Model in Stan
%https://rfarouni.github.io/assets/projects/BayesianFactorAnalysis/BayesianFactorAnalysis.html


% Idea Ruben: Use Trigonometric functions to set up prior that satisfies Trace restriction.
% \begin{itemize}
%     \item Use that $\cos^2{\theta}+\sin^2{\theta}=1$ and expand as follows
%     \begin{align}
%         J \cos^2{\theta_1}+J\sin^2{\theta_1}=J\\
%         J \cos^2{\theta_1}+J\sin^2{\theta_1}[ \cos^2{\theta_2}+\sin^2{\theta_2}]=J\\
%         J \cos^2{\theta_1}+J\sin^2{\theta_1}[ \cos^2{\theta_2}+\sin^2{\theta_2}[ \cos^2{\theta_3}+\sin^2{\theta_3}]]=J,
%     \end{align}
%     and put priors on $\theta_j$. For instance:
%     \begin{align}
%         \theta_j\sim \pi\Phi(\kappa_j),\quad \kappa_j\sim\mathcal{N}(0,\sigma^2),
%     \end{align}
%     where $\Phi$ is the cdf of a Gaussian distribution. 
% \item Shrink $\Sigma$ to identity matrix: set prior mean $\gamma=0$ and $D=I_J$. Since $\cos{\frac{\pi}{2}}=0$, $\sin{\frac{\pi}{2}}=1$, and for $\theta=\arctan{\sqrt{a}}$ it holds that $a\cos^2{\theta}=\sin^2{\theta}$, we have that $\Sigma=I_J$ if $\theta_j=\frac{\pi}{2}$ for $j=1,\dots,J\times q$ and $\theta_j=\arctan{\sqrt{J(q+1)-j}}$ for $j=J\times q,\dots,J\times q +J-1$.
% \item Von Mises distribution? Works well. But have to do similar trick with variance as for mean. 
% \item Conjugate priors. %https://en.wikipedia.org/wiki/Von_Mises_distribution
% %https://www.sciencedirect.com/science/article/pii/S0378375812003448
%     \end{itemize}
